Cosmological de Sitter Solutions of the Semiclassical Einstein Equation

Exponentially expanding space-times play a central role in contemporary cosmology, most importantly in the theory of inflation and in the Dark Energy driven expansion in the late universe. In this work, we give a complete list of de Sitter solutions of the semiclassical Einstein equation (SCE), where classical gravity is coupled to the expected value of a renormalized stress-energy tensor of a free quantum field in the Bunch-Davies state. To achieve this, we explicitly determine the stress-energy tensor associated with the Bunch-Davies state using the recently proposed `moment approach' on the cosmological coordinate patch of de Sitter space. From the energy component of the SCE we thus obtain an analytic consistency equation for the model's parameters which has to be fulfilled by solutions to the SCE. Using this equation we then investigate the number of solutions and the structure of the solution set in dependency on the coupling parameter of the quantum field to the scalar curvature and renormalization constants using analytic arguments in combination with numerical evidence. We also identify parameter sets where multiple expansion rates separated by several orders of magnitude are possible. Potentially for such parameter settings, a fast (semi-stable) expansion in the early universe could be compatible with a late time `Dark Energy-like' behavior of the universe.

==> Digammaplot.tex <==
\addplot[mark=none] coordinates {
   (    0.0500   ,  -59.2986   )
   (    0.0600   ,  -49.2942   )
   (    0.0700   ,  -42.1469   )
   (    0.0800   ,  -36.7854   )
   (    0.0900   ,  -32.6143   )
   (    0.1000   ,  -29.2766   )
   (    0.1100   ,  -26.5450   )
   (    0.1200   ,  -24.2679   )
   (    0.1300   ,  -22.3405   )
   (    0.1400   ,  -20.6878   )
   (    0.1500   ,  -19.2549   )
   (    0.1600   ,  -18.0007   )
   (    0.1700   ,  -16.8935   )
   (    0.1800   ,  -15.9088   )
   (    0.1900   ,  -15.0274   )
   (    0.2000   ,  -14.2337   )
   (    0.2100   ,  -13.5152   )
   (    0.2200   ,  -12.8617   )
   (    0.2300   ,  -12.2646   )
   (    0.2400   ,  -11.7170   )
   (    0.2500   ,  -11.2128   )
   (    0.2600   ,  -10.7472   )
   (    0.2700   ,  -10.3157   )
   (    0.2800   ,   -9.9148   )
   (    0.2900   ,   -9.5413   )
   (    0.3000   ,   -9.1924   )
   (    0.3100   ,   -8.8657   )
   (    0.3200   ,   -8.5593   )
   (    0.3300   ,   -8.2711   )
   (    0.3400   ,   -7.9998   )
   (    0.3500   ,   -7.7437   )
   (    0.3600   ,   -7.5016   )
   (    0.3700   ,   -7.2724   )
   (    0.3800   ,   -7.0551   )
   (    0.3900   ,   -6.8487   )
   (    0.4000   ,   -6.6524   )
   (    0.4100   ,   -6.4656   )
   (    0.4200   ,   -6.2875   )
   (    0.4300   ,   -6.1175   )
   (    0.4400   ,   -5.9550   )
   (    0.4500   ,   -5.7997   )
   (    0.4600   ,   -5.6509   )
   (    0.4700   ,   -5.5083   )
   (    0.4800   ,   -5.3715   )
   (    0.4900   ,   -5.2401   )
   (    0.5000   ,   -5.1139   )
   (    0.5100   ,   -4.9924   )
   (    0.5200   ,   -4.8755   )
   (    0.5300   ,   -4.7629   )
   (    0.5400   ,   -4.6544   )
   (    0.5500   ,   -4.5496   )
   (    0.5600   ,   -4.4485   )
   (    0.5700   ,   -4.3508   )
   (    0.5800   ,   -4.2564   )
   (    0.5900   ,   -4.1650   )
   (    0.6000   ,   -4.0766   )
   (    0.6100   ,   -3.9909   )
   (    0.6200   ,   -3.9080   )
   (    0.6300   ,   -3.8275   )
   (    0.6400   ,   -3.7495   )
   (    0.6500   ,   -3.6738   )
   (    0.6600   ,   -3.6002   )
   (    0.6700   ,   -3.5288   )
   (    0.6800   ,   -3.4594   )
   (    0.6900   ,   -3.3919   )
   (    0.7000   ,   -3.3262   )
   (    0.7100   ,   -3.2623   )
   (    0.7200   ,   -3.2000   )
   (    0.7300   ,   -3.1394   )
   (    0.7400   ,   -3.0804   )
   (    0.7500   ,   -3.0228   )
   (    0.7600   ,   -2.9667   )
   (    0.7700   ,   -2.9120   )
   (    0.7800   ,   -2.8585   )
   (    0.7900   ,   -2.8064   )
   (    0.8000   ,   -2.7555   )
   (    0.8100   ,   -2.7057   )
   (    0.8200   ,   -2.6571   )
   (    0.8300   ,   -2.6096   )
   (    0.8400   ,   -2.5632   )
   (    0.8500   ,   -2.5178   )
   (    0.8600   ,   -2.4734   )
   (    0.8700   ,   -2.4299   )
   (    0.8800   ,   -2.3873   )
   (    0.8900   ,   -2.3457   )
   (    0.9000   ,   -2.3049   )
   (    0.9100   ,   -2.2649   )
   (    0.9200   ,   -2.2258   )
   (    0.9300   ,   -2.1874   )
   (    0.9400   ,   -2.1498   )
   (    0.9500   ,   -2.1129   )
   (    0.9600   ,   -2.0767   )
   (    0.9700   ,   -2.0412   )
   (    0.9800   ,   -2.0064   )
   (    0.9900   ,   -1.9722   )
   (    1.0000   ,   -1.9386   )
   (    1.0100   ,   -1.9057   )
   (    1.0200   ,   -1.8733   )
   (    1.0300   ,   -1.8416   )
   (    1.0400   ,   -1.8103   )
   (    1.0500   ,   -1.7797   )
   (    1.0600   ,   -1.7495   )
   (    1.0700   ,   -1.7199   )
   (    1.0800   ,   -1.6907   )
   (    1.0900   ,   -1.6621   )
   (    1.1000   ,   -1.6339   )
   (    1.1100   ,   -1.6062   )
   (    1.1200   ,   -1.5789   )
   (    1.1300   ,   -1.5521   )
   (    1.1400   ,   -1.5257   )
   (    1.1500   ,   -1.4997   )
   (    1.1600   ,   -1.4741   )
   (    1.1700   ,   -1.4489   )
   (    1.1800   ,   -1.4241   )
   (    1.1900   ,   -1.3996   )
   (    1.2000   ,   -1.3756   )
   (    1.2100   ,   -1.3518   )
   (    1.2200   ,   -1.3285   )
   (    1.2300   ,   -1.3054   )
   (    1.2400   ,   -1.2827   )
   (    1.2500   ,   -1.2604   )
   (    1.2600   ,   -1.2383   )
   (    1.2700   ,   -1.2165   )
   (    1.2800   ,   -1.1951   )
   (    1.2900   ,   -1.1739   )
   (    1.3000   ,   -1.1530   )
   (    1.3100   ,   -1.1324   )
   (    1.3200   ,   -1.1121   )
   (    1.3300   ,   -1.0921   )
   (    1.3400   ,   -1.0723   )
   (    1.3500   ,   -1.0528   )
   (    1.3600   ,   -1.0335   )
   (    1.3700   ,   -1.0145   )
   (    1.3800   ,   -0.9957   )
   (    1.3900   ,   -0.9771   )
   (    1.4000   ,   -0.9588   )
   (    1.4100   ,   -0.9407   )
   (    1.4200   ,   -0.9228   )
   (    1.4300   ,   -0.9052   )
   (    1.4400   ,   -0.8877   )
   (    1.4500   ,   -0.8705   )
   (    1.4600   ,   -0.8535   )
   (    1.4700   ,   -0.8366   )
   (    1.4800   ,   -0.8200   )
   (    1.4900   ,   -0.8035   )
   (    1.5000   ,   -0.7873   )
   (    1.5100   ,   -0.7712   )
   (    1.5200   ,   -0.7553   )
   (    1.5300   ,   -0.7396   )
   (    1.5400   ,   -0.7241   )
   (    1.5500   ,   -0.7087   )
   (    1.5600   ,   -0.6935   )
   (    1.5700   ,   -0.6785   )
   (    1.5800   ,   -0.6636   )
   (    1.5900   ,   -0.6489   )
   (    1.6000   ,   -0.6344   )
   (    1.6100   ,   -0.6200   )
   (    1.6200   ,   -0.6057   )
   (    1.6300   ,   -0.5916   )
   (    1.6400   ,   -0.5777   )
   (    1.6500   ,   -0.5639   )
   (    1.6600   ,   -0.5502   )
   (    1.6700   ,   -0.5367   )
   (    1.6800   ,   -0.5233   )
   (    1.6900   ,   -0.5100   )
   (    1.7000   ,   -0.4969   )
   (    1.7100   ,   -0.4839   )
   (    1.7200   ,   -0.4710   )
   (    1.7300   ,   -0.4582   )
   (    1.7400   ,   -0.4456   )
   (    1.7500   ,   -0.4331   )
   (    1.7600   ,   -0.4207   )
   (    1.7700   ,   -0.4084   )
   (    1.7800   ,   -0.3963   )
   (    1.7900   ,   -0.3842   )
   (    1.8000   ,   -0.3723   )
   (    1.8100   ,   -0.3605   )
   (    1.8200   ,   -0.3488   )
   (    1.8300   ,   -0.3371   )
   (    1.8400   ,   -0.3256   )
   (    1.8500   ,   -0.3142   )
   (    1.8600   ,   -0.3029   )
   (    1.8700   ,   -0.2917   )
   (    1.8800   ,   -0.2806   )
   (    1.8900   ,   -0.2696   )
   (    1.9000   ,   -0.2587   )
   (    1.9100   ,   -0.2479   )
   (    1.9200   ,   -0.2371   )
   (    1.9300   ,   -0.2265   )
   (    1.9400   ,   -0.2159   )
   (    1.9500   ,   -0.2055   )
   (    1.9600   ,   -0.1951   )
   (    1.9700   ,   -0.1848   )
   (    1.9800   ,   -0.1746   )
   (    1.9900   ,   -0.1645   )
   (    2.0000   ,   -0.1544   )
   (    2.0100   ,   -0.1445   )
   (    2.0200   ,   -0.1346   )
   (    2.0300   ,   -0.1248   )
   (    2.0400   ,   -0.1151   )
   (    2.0500   ,   -0.1054   )
   (    2.0600   ,   -0.0958   )
   (    2.0700   ,   -0.0863   )
   (    2.0800   ,   -0.0769   )
   (    2.0900   ,   -0.0676   )
   (    2.1000   ,   -0.0583   )
   (    2.1100   ,   -0.0491   )
   (    2.1200   ,   -0.0399   )
   (    2.1300   ,   -0.0309   )
   (    2.1400   ,   -0.0219   )
   (    2.1500   ,   -0.0129   )
   (    2.1600   ,   -0.0040   )
   (    2.1700   ,    0.0048   )
   (    2.1800   ,    0.0135   )
   (    2.1900   ,    0.0222   )
   (    2.2000   ,    0.0308   )
   (    2.2100   ,    0.0394   )
   (    2.2200   ,    0.0479   )
   (    2.2300   ,    0.0563   )
   (    2.2400   ,    0.0647   )
   (    2.2500   ,    0.0730   )
   (    2.2600   ,    0.0812   )
   (    2.2700   ,    0.0894   )
   (    2.2800   ,    0.0976   )
   (    2.2900   ,    0.1057   )
   (    2.3000   ,    0.1137   )
   (    2.3100   ,    0.1217   )
   (    2.3200   ,    0.1296   )
   (    2.3300   ,    0.1375   )
   (    2.3400   ,    0.1453   )
   (    2.3500   ,    0.1531   )
   (    2.3600   ,    0.1608   )
   (    2.3700   ,    0.1685   )
   (    2.3800   ,    0.1761   )
   (    2.3900   ,    0.1836   )
   (    2.4000   ,    0.1912   )
   (    2.4100   ,    0.1986   )
   (    2.4200   ,    0.2061   )
   (    2.4300   ,    0.2134   )
   (    2.4400   ,    0.2208   )
   (    2.4500   ,    0.2280   )
   (    2.4600   ,    0.2353   )
   (    2.4700   ,    0.2425   )
   (    2.4800   ,    0.2496   )
   (    2.4900   ,    0.2567   )
   (    2.5000   ,    0.2638   )
   (    2.5100   ,    0.2708   )
   (    2.5200   ,    0.2778   )
   (    2.5300   ,    0.2847   )
   (    2.5400   ,    0.2916   )
   (    2.5500   ,    0.2984   )
   (    2.5600   ,    0.3053   )
   (    2.5700   ,    0.3120   )
   (    2.5800   ,    0.3187   )
   (    2.5900   ,    0.3254   )
   (    2.6000   ,    0.3321   )
   (    2.6100   ,    0.3387   )
   (    2.6200   ,    0.3453   )
   (    2.6300   ,    0.3518   )
   (    2.6400   ,    0.3583   )
   (    2.6500   ,    0.3648   )
   (    2.6600   ,    0.3712   )
   (    2.6700   ,    0.3776   )
   (    2.6800   ,    0.3839   )
   (    2.6900   ,    0.3902   )
   (    2.7000   ,    0.3965   )
   (    2.7100   ,    0.4028   )
   (    2.7200   ,    0.4090   )
   (    2.7300   ,    0.4151   )
   (    2.7400   ,    0.4213   )
   (    2.7500   ,    0.4274   )
   (    2.7600   ,    0.4335   )
   (    2.7700   ,    0.4395   )
   (    2.7800   ,    0.4455   )
   (    2.7900   ,    0.4515   )
   (    2.8000   ,    0.4575   )
   (    2.8100   ,    0.4634   )
   (    2.8200   ,    0.4692   )
   (    2.8300   ,    0.4751   )
   (    2.8400   ,    0.4809   )
   (    2.8500   ,    0.4867   )
   (    2.8600   ,    0.4925   )
   (    2.8700   ,    0.4982   )
   (    2.8800   ,    0.5039   )
   (    2.8900   ,    0.5096   )
   (    2.9000   ,    0.5152   )
   (    2.9100   ,    0.5208   )
   (    2.9200   ,    0.5264   )
   (    2.9300   ,    0.5320   )
   (    2.9400   ,    0.5375   )
   (    2.9500   ,    0.5430   )
   (    2.9600   ,    0.5485   )
   (    2.9700   ,    0.5540   )
   (    2.9800   ,    0.5594   )
   (    2.9900   ,    0.5648   )
   (    3.0000   ,    0.5701   )
   (    3.0100   ,    0.5755   )
   (    3.0200   ,    0.5808   )
   (    3.0300   ,    0.5861   )
   (    3.0400   ,    0.5914   )
   (    3.0500   ,    0.5966   )
   (    3.0600   ,    0.6018   )
   (    3.0700   ,    0.6070   )
   (    3.0800   ,    0.6122   )
   (    3.0900   ,    0.6173   )
   (    3.1000   ,    0.6224   )
   (    3.1100   ,    0.6275   )
   (    3.1200   ,    0.6326   )
   (    3.1300   ,    0.6377   )
   (    3.1400   ,    0.6427   )
   (    3.1500   ,    0.6477   )
   (    3.1600   ,    0.6527   )
   (    3.1700   ,    0.6576   )
   (    3.1800   ,    0.6626   )
   (    3.1900   ,    0.6675   )
   (    3.2000   ,    0.6724   )
   (    3.2100   ,    0.6772   )
   (    3.2200   ,    0.6821   )
   (    3.2300   ,    0.6869   )
   (    3.2400   ,    0.6917   )
   (    3.2500   ,    0.6965   )
   (    3.2600   ,    0.7012   )
   (    3.2700   ,    0.7060   )
   (    3.2800   ,    0.7107   )
   (    3.2900   ,    0.7154   )
   (    3.3000   ,    0.7201   )
   (    3.3100   ,    0.7247   )
   (    3.3200   ,    0.7294   )
   (    3.3300   ,    0.7340   )
   (    3.3400   ,    0.7386   )
   (    3.3500   ,    0.7432   )
   (    3.3600   ,    0.7477   )
   (    3.3700   ,    0.7523   )
   (    3.3800   ,    0.7568   )
   (    3.3900   ,    0.7613   )
   (    3.4000   ,    0.7658   )
   (    3.4100   ,    0.7702   )
   (    3.4200   ,    0.7747   )
   (    3.4300   ,    0.7791   )
   (    3.4400   ,    0.7835   )
   (    3.4500   ,    0.7879   )
   (    3.4600   ,    0.7923   )
   (    3.4700   ,    0.7966   )
   (    3.4800   ,    0.8010   )
   (    3.4900   ,    0.8053   )
   (    3.5000   ,    0.8096   )
   (    3.5100   ,    0.8139   )
   (    3.5200   ,    0.8181   )
   (    3.5300   ,    0.8224   )
   (    3.5400   ,    0.8266   )
   (    3.5500   ,    0.8309   )
   (    3.5600   ,    0.8351   )
   (    3.5700   ,    0.8392   )
   (    3.5800   ,    0.8434   )
   (    3.5900   ,    0.8476   )
   (    3.6000   ,    0.8517   )
   (    3.6100   ,    0.8558   )
   (    3.6200   ,    0.8599   )
   (    3.6300   ,    0.8640   )
   (    3.6400   ,    0.8681   )
   (    3.6500   ,    0.8721   )
   (    3.6600   ,    0.8762   )
   (    3.6700   ,    0.8802   )
   (    3.6800   ,    0.8842   )
   (    3.6900   ,    0.8882   )
   (    3.7000   ,    0.8922   )
   (    3.7100   ,    0.8962   )
   (    3.7200   ,    0.9001   )
   (    3.7300   ,    0.9040   )
   (    3.7400   ,    0.9080   )
   (    3.7500   ,    0.9119   )
   (    3.7600   ,    0.9158   )
   (    3.7700   ,    0.9196   )
   (    3.7800   ,    0.9235   )
   (    3.7900   ,    0.9274   )
   (    3.8000   ,    0.9312   )
   (    3.8100   ,    0.9350   )
   (    3.8200   ,    0.9388   )
   (    3.8300   ,    0.9426   )
   (    3.8400   ,    0.9464   )
   (    3.8500   ,    0.9502   )
   (    3.8600   ,    0.9539   )
   (    3.8700   ,    0.9577   )
   (    3.8800   ,    0.9614   )
   (    3.8900   ,    0.9651   )
   (    3.9000   ,    0.9688   )
   (    3.9100   ,    0.9725   )
   (    3.9200   ,    0.9762   )
   (    3.9300   ,    0.9798   )
   (    3.9400   ,    0.9835   )
   (    3.9500   ,    0.9871   )
   (    3.9600   ,    0.9908   )
   (    3.9700   ,    0.9944   )
   (    3.9800   ,    0.9980   )
   (    3.9900   ,    1.0016   )
   (    4.0000   ,    1.0051   )
   (    4.0100   ,    1.0087   )
   (    4.0200   ,    1.0123   )
   (    4.0300   ,    1.0158   )
   (    4.0400   ,    1.0193   )
   (    4.0500   ,    1.0228   )
   (    4.0600   ,    1.0263   )
   (    4.0700   ,    1.0298   )
   (    4.0800   ,    1.0333   )
   (    4.0900   ,    1.0368   )
   (    4.1000   ,    1.0402   )
   (    4.1100   ,    1.0437   )
   (    4.1200   ,    1.0471   )
   (    4.1300   ,    1.0506   )
   (    4.1400   ,    1.0540   )
   (    4.1500   ,    1.0574   )
   (    4.1600   ,    1.0608   )
   (    4.1700   ,    1.0641   )
   (    4.1800   ,    1.0675   )
   (    4.1900   ,    1.0709   )
   (    4.2000   ,    1.0742   )
   (    4.2100   ,    1.0776   )
   (    4.2200   ,    1.0809   )
   (    4.2300   ,    1.0842   )
   (    4.2400   ,    1.0875   )
   (    4.2500   ,    1.0908   )
   (    4.2600   ,    1.0941   )
   (    4.2700   ,    1.0973   )
   (    4.2800   ,    1.1006   )
   (    4.2900   ,    1.1039   )
   (    4.3000   ,    1.1071   )
   (    4.3100   ,    1.1103   )
   (    4.3200   ,    1.1136   )
   (    4.3300   ,    1.1168   )
   (    4.3400   ,    1.1200   )
   (    4.3500   ,    1.1232   )
   (    4.3600   ,    1.1264   )
   (    4.3700   ,    1.1295   )
   (    4.3800   ,    1.1327   )
   (    4.3900   ,    1.1359   )
   (    4.4000   ,    1.1390   )
   (    4.4100   ,    1.1421   )
   (    4.4200   ,    1.1453   )
   (    4.4300   ,    1.1484   )
   (    4.4400   ,    1.1515   )
   (    4.4500   ,    1.1546   )
   (    4.4600   ,    1.1577   )
   (    4.4700   ,    1.1608   )
   (    4.4800   ,    1.1638   )
   (    4.4900   ,    1.1669   )
   (    4.5000   ,    1.1699   )
   (    4.5100   ,    1.1730   )
   (    4.5200   ,    1.1760   )
   (    4.5300   ,    1.1790   )
   (    4.5400   ,    1.1821   )
   (    4.5500   ,    1.1851   )
   (    4.5600   ,    1.1881   )
   (    4.5700   ,    1.1911   )
   (    4.5800   ,    1.1940   )
   (    4.5900   ,    1.1970   )
   (    4.6000   ,    1.2000   )
   (    4.6100   ,    1.2029   )
   (    4.6200   ,    1.2059   )
   (    4.6300   ,    1.2088   )
   (    4.6400   ,    1.2118   )
   (    4.6500   ,    1.2147   )
   (    4.6600   ,    1.2176   )
   (    4.6700   ,    1.2205   )
   (    4.6800   ,    1.2234   )
   (    4.6900   ,    1.2263   )
   (    4.7000   ,    1.2292   )
   (    4.7100   ,    1.2321   )
   (    4.7200   ,    1.2349   )
   (    4.7300   ,    1.2378   )
   (    4.7400   ,    1.2406   )
   (    4.7500   ,    1.2435   )
   (    4.7600   ,    1.2463   )
   (    4.7700   ,    1.2491   )
   (    4.7800   ,    1.2520   )
   (    4.7900   ,    1.2548   )
   (    4.8000   ,    1.2576   )
   (    4.8100   ,    1.2604   )
   (    4.8200   ,    1.2632   )
   (    4.8300   ,    1.2659   )
   (    4.8400   ,    1.2687   )
   (    4.8500   ,    1.2715   )
   (    4.8600   ,    1.2742   )
   (    4.8700   ,    1.2770   )
   (    4.8800   ,    1.2797   )
   (    4.8900   ,    1.2825   )
   (    4.9000   ,    1.2852   )
   (    4.9100   ,    1.2879   )
   (    4.9200   ,    1.2906   )
   (    4.9300   ,    1.2933   )
   (    4.9400   ,    1.2961   )
   (    4.9500   ,    1.2987   )
   (    4.9600   ,    1.3014   )
   (    4.9700   ,    1.3041   )
   (    4.9800   ,    1.3068   )
   (    4.9900   ,    1.3095   )
   (    5.0000   ,    1.3121   )
};

==> Digammaplot2.tex <==
\addplot[mark=none] coordinates {
   (  -39.9000   , -126.1784   )
   (  -39.8000   ,  -61.1554   )
   (  -39.7000   ,  -39.4657   )
   (  -39.6000   ,  -28.6093   )
   (  -39.5000   ,  -22.0862   )
   (  -39.4000   ,  -17.7297   )
   (  -39.3000   ,  -14.6113   )
   (  -39.2000   ,  -12.2666   )
   (  -39.1000   ,  -10.4376   )
   (  -39.0000   ,   -8.9698   )
   (  -38.9000   ,   -7.7644   )
   (  -38.8000   ,   -6.7559   )
   (  -38.7000   ,   -5.8989   )
   (  -38.6000   ,   -5.1608   )
   (  -38.5000   ,   -4.5178   )
   (  -38.4000   ,   -3.9520   )
   (  -38.3000   ,   -3.4499   )
   (  -38.2000   ,   -3.0007   )
   (  -38.1000   ,   -2.5961   )
   (  -38.0000   ,   -2.2293   )
   (  -37.9000   ,   -1.8950   )
   (  -37.8000   ,   -1.5886   )
   (  -37.7000   ,   -1.3066   )
   (  -37.6000   ,   -1.0457   )
   (  -37.5000   ,   -0.8035   )
   (  -37.4000   ,   -0.5777   )
   (  -37.3000   ,   -0.3666   )
   (  -37.2000   ,   -0.1684   )
   (  -37.1000   ,    0.0181   )
   (  -37.0000   ,    0.1943   )
   (  -36.9000   ,    0.3610   )
   (  -36.8000   ,    0.5193   )
   (  -36.7000   ,    0.6699   )
   (  -36.6000   ,    0.8136   )
   (  -36.5000   ,    0.9510   )
   (  -36.4000   ,    1.0826   )
   (  -36.3000   ,    1.2090   )
   (  -36.2000   ,    1.3307   )
   (  -36.1000   ,    1.4479   )
   (  -36.0000   ,    1.5612   )
   (  -35.9000   ,    1.6708   )
   (  -35.8000   ,    1.7770   )
   (  -35.7000   ,    1.8802   )
   (  -35.6000   ,    1.9806   )
   (  -35.5000   ,    2.0784   )
   (  -35.4000   ,    2.1739   )
   (  -35.3000   ,    2.2672   )
   (  -35.2000   ,    2.3586   )
   (  -35.1000   ,    2.4482   )
   (  -35.0000   ,    2.5362   )
   (  -34.9000   ,    2.6228   )
   (  -34.8000   ,    2.7080   )
   (  -34.7000   ,    2.7921   )
   (  -34.6000   ,    2.8752   )
   (  -34.5000   ,    2.9574   )
   (  -34.4000   ,    3.0388   )
   (  -34.3000   ,    3.1196   )
   (  -34.2000   ,    3.1999   )
   (  -34.1000   ,    3.2798   )
   (  -34.0000   ,    3.3594   )
   (  -33.9000   ,    3.4388   )
   (  -33.8000   ,    3.5182   )
   (  -33.7000   ,    3.5976   )
   (  -33.6000   ,    3.6771   )
   (  -33.5000   ,    3.7570   )
   (  -33.4000   ,    3.8372   )
   (  -33.3000   ,    3.9180   )
   (  -33.2000   ,    3.9993   )
   (  -33.1000   ,    4.0815   )
   (  -33.0000   ,    4.1645   )
   (  -32.9000   ,    4.2486   )
   (  -32.8000   ,    4.3338   )
   (  -32.7000   ,    4.4204   )
   (  -32.6000   ,    4.5084   )
   (  -32.5000   ,    4.5981   )
   (  -32.4000   ,    4.6897   )
   (  -32.3000   ,    4.7833   )
   (  -32.2000   ,    4.8791   )
   (  -32.1000   ,    4.9773   )
   (  -32.0000   ,    5.0783   )
   (  -31.9000   ,    5.1823   )
   (  -31.8000   ,    5.2895   )
   (  -31.7000   ,    5.4003   )
   (  -31.6000   ,    5.5151   )
   (  -31.5000   ,    5.6342   )
   (  -31.4000   ,    5.7581   )
   (  -31.3000   ,    5.8872   )
   (  -31.2000   ,    6.0221   )
   (  -31.1000   ,    6.1634   )
   (  -31.0000   ,    6.3118   )
   (  -30.9000   ,    6.4681   )
   (  -30.8000   ,    6.6332   )
   (  -30.7000   ,    6.8080   )
   (  -30.6000   ,    6.9937   )
   (  -30.5000   ,    7.1918   )
   (  -30.4000   ,    7.4038   )
   (  -30.3000   ,    7.6314   )
   (  -30.2000   ,    7.8770   )
   (  -30.1000   ,    8.1432   )
   (  -30.0000   ,    8.4329   )
   (  -29.9000   ,    8.7501   )
   (  -29.8000   ,    9.0993   )
   (  -29.7000   ,    9.4862   )
   (  -29.6000   ,    9.9178   )
   (  -29.5000   ,   10.4033   )
   (  -29.4000   ,   10.9542   )
   (  -29.3000   ,   11.5855   )
   (  -29.2000   ,   12.3175   )
   (  -29.1000   ,   13.1776   )
   (  -29.0000   ,   14.2043   )
   (  -28.9000   ,   15.4532   )
   (  -28.8000   ,   17.0076   )
   (  -28.7000   ,   18.9984   )
   (  -28.6000   ,   21.6440   )
   (  -28.5000   ,   25.3372   )
   (  -28.4000   ,   30.8637   )
   (  -28.3000   ,   40.0569   )
   (  -28.2000   ,   58.4167   )
   (  -28.1000   ,  113.4433   )
   };
\addplot[mark=none] coordinates {
   (  -27.9000   , -106.5036   )
   (  -27.8000   ,  -51.4769   )
   (  -27.7000   ,  -33.1169   )
   (  -27.6000   ,  -23.9235   )
   (  -27.5000   ,  -18.3966   )
   (  -27.4000   ,  -14.7030   )
   (  -27.3000   ,  -12.0569   )
   (  -27.2000   ,  -10.0655   )
   (  -27.1000   ,   -8.5105   )
   (  -27.0000   ,   -7.2608   )
   (  -26.9000   ,   -6.2333   )
   (  -26.8000   ,   -5.3722   )
   (  -26.7000   ,   -4.6392   )
   (  -26.6000   ,   -4.0068   )
   (  -26.5000   ,   -3.4547   )
   (  -26.4000   ,   -2.9679   )
   (  -26.3000   ,   -2.5348   )
   (  -26.2000   ,   -2.1464   )
   (  -26.1000   ,   -1.7956   )
   (  -26.0000   ,   -1.4767   )
   (  -25.9000   ,   -1.1851   )
   (  -25.8000   ,   -0.9170   )
   (  -25.7000   ,   -0.6692   )
   (  -25.6000   ,   -0.4393   )
   (  -25.5000   ,   -0.2249   )
   (  -25.4000   ,   -0.0243   )
   (  -25.3000   ,    0.1642   )
   (  -25.2000   ,    0.3419   )
   (  -25.1000   ,    0.5100   )
   (  -25.0000   ,    0.6696   )
   (  -24.9000   ,    0.8214   )
   (  -24.8000   ,    0.9664   )
   (  -24.7000   ,    1.1052   )
   (  -24.6000   ,    1.2384   )
   (  -24.5000   ,    1.3667   )
   (  -24.4000   ,    1.4904   )
   (  -24.3000   ,    1.6101   )
   (  -24.2000   ,    1.7261   )
   (  -24.1000   ,    1.8388   )
   (  -24.0000   ,    1.9487   )
   (  -23.9000   ,    2.0559   )
   (  -23.8000   ,    2.1607   )
   (  -23.7000   ,    2.2635   )
   (  -23.6000   ,    2.3645   )
   (  -23.5000   ,    2.4640   )
   (  -23.4000   ,    2.5621   )
   (  -23.3000   ,    2.6591   )
   (  -23.2000   ,    2.7552   )
   (  -23.1000   ,    2.8506   )
   (  -23.0000   ,    2.9455   )
   (  -22.9000   ,    3.0401   )
   (  -22.8000   ,    3.1345   )
   (  -22.7000   ,    3.2291   )
   (  -22.6000   ,    3.3239   )
   (  -22.5000   ,    3.4192   )
   (  -22.4000   ,    3.5152   )
   (  -22.3000   ,    3.6121   )
   (  -22.2000   ,    3.7101   )
   (  -22.1000   ,    3.8094   )
   (  -22.0000   ,    3.9104   )
   (  -21.9000   ,    4.0131   )
   (  -21.8000   ,    4.1180   )
   (  -21.7000   ,    4.2253   )
   (  -21.6000   ,    4.3353   )
   (  -21.5000   ,    4.4484   )
   (  -21.4000   ,    4.5649   )
   (  -21.3000   ,    4.6854   )
   (  -21.2000   ,    4.8102   )
   (  -21.1000   ,    4.9398   )
   (  -21.0000   ,    5.0749   )
   (  -20.9000   ,    5.2161   )
   (  -20.8000   ,    5.3642   )
   (  -20.7000   ,    5.5200   )
   (  -20.6000   ,    5.6845   )
   (  -20.5000   ,    5.8588   )
   (  -20.4000   ,    6.0442   )
   (  -20.3000   ,    6.2422   )
   (  -20.2000   ,    6.4547   )
   (  -20.1000   ,    6.6838   )
   (  -20.0000   ,    6.9321   )
   (  -19.9000   ,    7.2026   )
   (  -19.8000   ,    7.4991   )
   (  -19.7000   ,    7.8264   )
   (  -19.6000   ,    8.1901   )
   (  -19.5000   ,    8.5978   )
   (  -19.4000   ,    9.0588   )
   (  -19.3000   ,    9.5856   )
   (  -19.2000   ,   10.1946   )
   (  -19.1000   ,   10.9084   )
   (  -19.0000   ,   11.7584   )
   (  -18.9000   ,   12.7901   )
   (  -18.8000   ,   14.0717   )
   (  -18.7000   ,   15.7104   )
   (  -18.6000   ,   17.8847   )
   (  -18.5000   ,   20.9162   )
   (  -18.4000   ,   25.4476   )
   (  -18.3000   ,   32.9790   )
   (  -18.2000   ,   48.0104   )
   (  -18.1000   ,   93.0419   )
   };
\addplot[mark=none] coordinates {
   (  -17.9000   ,  -86.8951   )
   (  -17.8000   ,  -41.8635   )
   (  -17.7000   ,  -26.8317   )
   (  -17.6000   ,  -19.2999   )
   (  -17.5000   ,  -14.7678   )
   (  -17.4000   ,  -11.7357   )
   (  -17.3000   ,   -9.5605   )
   (  -17.2000   ,   -7.9208   )
   (  -17.1000   ,   -6.6380   )
   (  -17.0000   ,   -5.6050   )
   (  -16.9000   ,   -4.7536   )
   (  -16.8000   ,   -4.0382   )
   (  -16.7000   ,   -3.4274   )
   (  -16.6000   ,   -2.8986   )
   (  -16.5000   ,   -2.4354   )
   (  -16.4000   ,   -2.0254   )
   (  -16.3000   ,   -1.6591   )
   (  -16.2000   ,   -1.3291   )
   (  -16.1000   ,   -1.0296   )
   (  -16.0000   ,   -0.7558   )
   (  -15.9000   ,   -0.5040   )
   (  -15.8000   ,   -0.2712   )
   (  -15.7000   ,   -0.0546   )
   (  -15.6000   ,    0.1479   )
   (  -15.5000   ,    0.3380   )
   (  -15.4000   ,    0.5174   )
   (  -15.3000   ,    0.6874   )
   (  -15.2000   ,    0.8491   )
   (  -15.1000   ,    1.0036   )
   (  -15.0000   ,    1.1517   )
   (  -14.9000   ,    1.2941   )
   (  -14.8000   ,    1.4318   )
   (  -14.7000   ,    1.5651   )
   (  -14.6000   ,    1.6948   )
   (  -14.5000   ,    1.8213   )
   (  -14.4000   ,    1.9451   )
   (  -14.3000   ,    2.0667   )
   (  -14.2000   ,    2.1866   )
   (  -14.1000   ,    2.3050   )
   (  -14.0000   ,    2.4225   )
   (  -13.9000   ,    2.5393   )
   (  -13.8000   ,    2.6559   )
   (  -13.7000   ,    2.7727   )
   (  -13.6000   ,    2.8900   )
   (  -13.5000   ,    3.0082   )
   (  -13.4000   ,    3.1278   )
   (  -13.3000   ,    3.2491   )
   (  -13.2000   ,    3.3727   )
   (  -13.1000   ,    3.4989   )
   (  -13.0000   ,    3.6284   )
   (  -12.9000   ,    3.7618   )
   (  -12.8000   ,    3.8996   )
   (  -12.7000   ,    4.0426   )
   (  -12.6000   ,    4.1916   )
   (  -12.5000   ,    4.3476   )
   (  -12.4000   ,    4.5116   )
   (  -12.3000   ,    4.6848   )
   (  -12.2000   ,    4.8687   )
   (  -12.1000   ,    5.0650   )
   (  -12.0000   ,    5.2757   )
   (  -11.9000   ,    5.5033   )
   (  -11.8000   ,    5.7507   )
   (  -11.7000   ,    6.0216   )
   (  -11.6000   ,    6.3206   )
   (  -11.5000   ,    6.6534   )
   (  -11.4000   ,    7.0274   )
   (  -11.3000   ,    7.4523   )
   (  -11.2000   ,    7.9410   )
   (  -11.1000   ,    8.5109   )
   (  -11.0000   ,    9.1865   )
   (  -10.9000   ,   10.0033   )
   (  -10.8000   ,   11.0144   )
   (  -10.7000   ,   12.3031   )
   (  -10.6000   ,   14.0083   )
   (  -10.5000   ,   16.3800   )
   (  -10.4000   ,   19.9183   )
   (  -10.3000   ,   25.7900   )
   (  -10.2000   ,   37.4950   )
   (  -10.1000   ,   72.5333   )
   };
\addplot[mark=none] coordinates {   
   (   -9.9000   ,  -67.3897   )
   (   -9.8000   ,  -32.3510   )
   (   -9.7000   ,  -20.6454   )
   (   -9.6000   ,  -14.7729   )
   (   -9.5000   ,  -11.2335   )
   (   -9.4000   ,   -8.8604   )
   (   -9.3000   ,   -7.1536   )
   (   -9.2000   ,   -5.8631   )
   (   -9.1000   ,   -4.8498   )
   (   -9.0000   ,   -4.0305   )
   (   -8.9000   ,   -3.3520   )
   (   -8.8000   ,   -2.7789   )
   (   -8.7000   ,   -2.2867   )
   (   -8.6000   ,   -1.8578   )
   (   -8.5000   ,   -1.4793   )
   (   -8.4000   ,   -1.1415   )
   (   -8.3000   ,   -0.8370   )
   (   -8.2000   ,   -0.5600   )
   (   -8.1000   ,   -0.3059   )
   (   -8.0000   ,   -0.0709   )
   (   -7.9000   ,    0.1481   )
   (   -7.8000   ,    0.3534   )
   (   -7.7000   ,    0.5474   )
   (   -7.6000   ,    0.7317   )
   (   -7.5000   ,    0.9079   )
   (   -7.4000   ,    1.0775   )
   (   -7.3000   ,    1.2416   )
   (   -7.2000   ,    1.4013   )
   (   -7.1000   ,    1.5577   )
   (   -7.0000   ,    1.7116   )
   (   -6.9000   ,    1.8641   )
   (   -6.8000   ,    2.0160   )
   (   -6.7000   ,    2.1682   )
   (   -6.6000   ,    2.3217   )
   (   -6.5000   ,    2.4773   )
   (   -6.4000   ,    2.6361   )
   (   -6.3000   ,    2.7993   )
   (   -6.2000   ,    2.9680   )
   (   -6.1000   ,    3.1437   )
   (   -6.0000   ,    3.3280   )
   (   -5.9000   ,    3.5227   )
   (   -5.8000   ,    3.7302   )
   (   -5.7000   ,    3.9532   )
   (   -5.6000   ,    4.1950   )
   (   -5.5000   ,    4.4599   )
   (   -5.4000   ,    4.7533   )
   (   -5.3000   ,    5.0822   )
   (   -5.2000   ,    5.4557   )
   (   -5.1000   ,    5.8866   )
   (   -5.0000   ,    6.3924   )
   (   -4.9000   ,    6.9984   )
   (   -4.8000   ,    7.7427   )
   (   -4.7000   ,    8.6848   )
   (   -4.6000   ,    9.9241   )
   (   -4.5000   ,   11.6392   )
   (   -4.4000   ,   14.1873   )
   (   -4.3000   ,   18.4019   )
   (   -4.2000   ,   26.7831   )
   (   -4.1000   ,   51.8310   )
   };
\addplot[mark=none] coordinates {
   (   -3.9000   ,  -48.0730   )
   (   -3.8000   ,  -23.0245   )
   (   -3.7000   ,  -14.6423   )
   (   -3.6000   ,  -10.4263   )
   (   -3.5000   ,   -7.8762   )
   (   -3.4000   ,   -6.1587   )
   (   -3.3000   ,   -4.9164   )
   (   -3.2000   ,   -3.9705   )
   (   -3.1000   ,   -3.2218   )
   (   -3.0000   ,   -2.6105   )
   (   -2.9000   ,   -2.0985   )
   (   -2.8000   ,   -1.6602   )
   (   -2.7000   ,   -1.2779   )
   (   -2.6000   ,   -0.9387   )
   (   -2.5000   ,   -0.6332   )
   (   -2.4000   ,   -0.3540   )
   (   -2.3000   ,   -0.0954   )
   (   -2.2000   ,    0.1474   )
   (   -2.1000   ,    0.3782   )
   (   -2.0000   ,    0.6006   )
   (   -1.9000   ,    0.8176   )
   (   -1.8000   ,    1.0323   )
   (   -1.7000   ,    1.2475   )
   (   -1.6000   ,    1.4665   )
   (   -1.5000   ,    1.6926   )
   (   -1.4000   ,    1.9299   )
   (   -1.3000   ,    2.1831   )
   (   -1.2000   ,    2.4585   )
   (   -1.1000   ,    2.7640   )
   (   -1.0000   ,    3.1107   )
   (   -0.9000   ,    3.5139   )
   (   -0.8000   ,    3.9969   )
   (   -0.7000   ,    4.5957   )
   (   -0.6000   ,    5.3700   )
   (   -0.5000   ,    6.4273   )
   (   -0.4000   ,    7.9820   )
   (   -0.3000   ,   10.5343   )
   (   -0.2000   ,   15.5845   )
   (   -0.1000   ,   30.6326   )
   };
\addplot[mark=none] coordinates {
   (    0.1000   ,  -29.2766   )
   (    0.2000   ,  -14.2337   )
   (    0.3000   ,   -9.1924   )
   (    0.4000   ,   -6.6524   )
   (    0.5000   ,   -5.1139   )
   (    0.6000   ,   -4.0766   )
   (    0.7000   ,   -3.3262   )
   (    0.8000   ,   -2.7555   )
   (    0.9000   ,   -2.3049   )
   (    1.0000   ,   -1.9386   )
   (    1.1000   ,   -1.6339   )
   (    1.2000   ,   -1.3756   )
   (    1.3000   ,   -1.1530   )
   (    1.4000   ,   -0.9588   )
   (    1.5000   ,   -0.7873   )
   (    1.6000   ,   -0.6344   )
   (    1.7000   ,   -0.4969   )
   (    1.8000   ,   -0.3723   )
   (    1.9000   ,   -0.2587   )
   (    2.0000   ,   -0.1544   )
   (    2.1000   ,   -0.0583   )
   (    2.2000   ,    0.0308   )
   (    2.3000   ,    0.1137   )
   (    2.4000   ,    0.1912   )
   (    2.5000   ,    0.2638   )
   (    2.6000   ,    0.3321   )
   (    2.7000   ,    0.3965   )
   (    2.8000   ,    0.4575   )
   (    2.9000   ,    0.5152   )
   (    3.0000   ,    0.5701   )
   (    3.1000   ,    0.6224   )
   (    3.2000   ,    0.6724   )
   (    3.3000   ,    0.7201   )
   (    3.4000   ,    0.7658   )
   (    3.5000   ,    0.8096   )
   (    3.6000   ,    0.8517   )
   (    3.7000   ,    0.8922   )
   (    3.8000   ,    0.9312   )
   (    3.9000   ,    0.9688   )
   (    4.0000   ,    1.0051   )
   (    4.1000   ,    1.0402   )
   (    4.2000   ,    1.0742   )
   (    4.3000   ,    1.1071   )
   (    4.4000   ,    1.1390   )
   (    4.5000   ,    1.1699   )
   (    4.6000   ,    1.2000   )
   (    4.7000   ,    1.2292   )
   (    4.8000   ,    1.2576   )
   (    4.9000   ,    1.2852   )
   (    5.0000   ,    1.3121   )
   (    5.1000   ,    1.3383   )
   (    5.2000   ,    1.3639   )
   (    5.3000   ,    1.3889   )
   (    5.4000   ,    1.4132   )
   (    5.5000   ,    1.4370   )
   (    5.6000   ,    1.4602   )
   (    5.7000   ,    1.4830   )
   (    5.8000   ,    1.5052   )
   (    5.9000   ,    1.5270   )
   (    6.0000   ,    1.5483   )
   (    6.1000   ,    1.5691   )
   (    6.2000   ,    1.5896   )
   (    6.3000   ,    1.6096   )
   (    6.4000   ,    1.6293   )
   (    6.5000   ,    1.6486   )
   (    6.6000   ,    1.6675   )
   (    6.7000   ,    1.6861   )
   (    6.8000   ,    1.7043   )
   (    6.9000   ,    1.7222   )
   (    7.0000   ,    1.7399   )
   (    7.1000   ,    1.7572   )
   (    7.2000   ,    1.7742   )
   (    7.3000   ,    1.7909   )
   (    7.4000   ,    1.8074   )
   (    7.5000   ,    1.8236   )
   (    7.6000   ,    1.8395   )
   (    7.7000   ,    1.8552   )
   (    7.8000   ,    1.8707   )
   (    7.9000   ,    1.8859   )
   (    8.0000   ,    1.9009   )
   (    8.1000   ,    1.9157   )
   (    8.2000   ,    1.9302   )
   (    8.3000   ,    1.9446   )
   (    8.4000   ,    1.9587   )
   (    8.5000   ,    1.9727   )
   (    8.6000   ,    1.9864   )
   (    8.7000   ,    2.0000   )
   (    8.8000   ,    2.0134   )
   (    8.9000   ,    2.0267   )
   (    9.0000   ,    2.0397   )
   (    9.1000   ,    2.0526   )
   (    9.2000   ,    2.0653   )
   (    9.3000   ,    2.0779   )
   (    9.4000   ,    2.0903   )
   (    9.5000   ,    2.1025   )
   (    9.6000   ,    2.1146   )
   (    9.7000   ,    2.1266   )
   (    9.8000   ,    2.1384   )
   (    9.9000   ,    2.1501   )
   (   10.0000   ,    2.1617   )
   (   10.1000   ,    2.1731   )
   (   10.2000   ,    2.1844   )
   (   10.3000   ,    2.1956   )
   (   10.4000   ,    2.2066   )
   (   10.5000   ,    2.2175   )
   (   10.6000   ,    2.2283   )
   (   10.7000   ,    2.2390   )
   (   10.8000   ,    2.2496   )
   (   10.9000   ,    2.2601   )
   (   11.0000   ,    2.2704   )
   (   11.1000   ,    2.2807   )
   (   11.2000   ,    2.2908   )
   (   11.3000   ,    2.3009   )
   (   11.4000   ,    2.3108   )
   (   11.5000   ,    2.3207   )
   (   11.6000   ,    2.3305   )
   (   11.7000   ,    2.3401   )
   (   11.8000   ,    2.3497   )
   (   11.9000   ,    2.3592   )
   (   12.0000   ,    2.3686   )
   (   12.1000   ,    2.3779   )
   (   12.2000   ,    2.3871   )
   (   12.3000   ,    2.3962   )
   (   12.4000   ,    2.4053   )
   (   12.5000   ,    2.4142   )
   (   12.6000   ,    2.4231   )
   (   12.7000   ,    2.4319   )
   (   12.8000   ,    2.4407   )
   (   12.9000   ,    2.4493   )
   (   13.0000   ,    2.4579   )
   (   13.1000   ,    2.4664   )
   (   13.2000   ,    2.4749   )
   (   13.3000   ,    2.4833   )
   (   13.4000   ,    2.4916   )
   (   13.5000   ,    2.4998   )
   (   13.6000   ,    2.5080   )
   (   13.7000   ,    2.5161   )
   (   13.8000   ,    2.5241   )
   (   13.9000   ,    2.5321   )
   (   14.0000   ,    2.5400   )
   (   14.1000   ,    2.5478   )
   (   14.2000   ,    2.5556   )
   (   14.3000   ,    2.5633   )
   (   14.4000   ,    2.5710   )
   (   14.5000   ,    2.5786   )
   (   14.6000   ,    2.5862   )
   (   14.7000   ,    2.5937   )
   (   14.8000   ,    2.6011   )
   (   14.9000   ,    2.6085   )
   (   15.0000   ,    2.6158   )
   (   15.1000   ,    2.6231   )
   (   15.2000   ,    2.6303   )
   (   15.3000   ,    2.6375   )
   (   15.4000   ,    2.6446   )
   (   15.5000   ,    2.6517   )
   (   15.6000   ,    2.6587   )
   (   15.7000   ,    2.6657   )
   (   15.8000   ,    2.6726   )
   (   15.9000   ,    2.6795   )
   (   16.0000   ,    2.6863   )
   (   16.1000   ,    2.6931   )
   (   16.2000   ,    2.6999   )
   (   16.3000   ,    2.7065   )
   (   16.4000   ,    2.7132   )
   (   16.5000   ,    2.7198   )
   (   16.6000   ,    2.7264   )
   (   16.7000   ,    2.7329   )
   (   16.8000   ,    2.7394   )
   (   16.9000   ,    2.7458   )
   (   17.0000   ,    2.7522   )
   (   17.1000   ,    2.7585   )
   (   17.2000   ,    2.7649   )
   (   17.3000   ,    2.7711   )
   (   17.4000   ,    2.7774   )
   (   17.5000   ,    2.7836   )
   (   17.6000   ,    2.7897   )
   (   17.7000   ,    2.7958   )
   (   17.8000   ,    2.8019   )
   (   17.9000   ,    2.8080   )
   (   18.0000   ,    2.8140   )
   (   18.1000   ,    2.8200   )
   (   18.2000   ,    2.8259   )
   (   18.3000   ,    2.8318   )
   (   18.4000   ,    2.8377   )
   (   18.5000   ,    2.8435   )
   (   18.6000   ,    2.8493   )
   (   18.7000   ,    2.8551   )
   (   18.8000   ,    2.8608   )
   (   18.9000   ,    2.8665   )
   (   19.0000   ,    2.8722   )
   (   19.1000   ,    2.8778   )
   (   19.2000   ,    2.8834   )
   (   19.3000   ,    2.8890   )
   (   19.4000   ,    2.8946   )
   (   19.5000   ,    2.9001   )
   (   19.6000   ,    2.9056   )
   (   19.7000   ,    2.9110   )
   (   19.8000   ,    2.9164   )
   (   19.9000   ,    2.9218   )
   (   20.0000   ,    2.9272   )
   (   20.1000   ,    2.9325   )
   (   20.2000   ,    2.9378   )
   (   20.3000   ,    2.9431   )
   (   20.4000   ,    2.9484   )
   (   20.5000   ,    2.9536   )
   (   20.6000   ,    2.9588   )
   (   20.7000   ,    2.9640   )
   (   20.8000   ,    2.9691   )
   (   20.9000   ,    2.9742   )
   (   21.0000   ,    2.9793   )
   (   21.1000   ,    2.9844   )
   (   21.2000   ,    2.9894   )
   (   21.3000   ,    2.9945   )
   (   21.4000   ,    2.9995   )
   (   21.5000   ,    3.0044   )
   (   21.6000   ,    3.0094   )
   (   21.7000   ,    3.0143   )
   (   21.8000   ,    3.0192   )
   (   21.9000   ,    3.0240   )
   (   22.0000   ,    3.0289   )
   (   22.1000   ,    3.0337   )
   (   22.2000   ,    3.0385   )
   (   22.3000   ,    3.0433   )
   (   22.4000   ,    3.0481   )
   (   22.5000   ,    3.0528   )
   (   22.6000   ,    3.0575   )
   (   22.7000   ,    3.0622   )
   (   22.8000   ,    3.0668   )
   (   22.9000   ,    3.0715   )
   (   23.0000   ,    3.0761   )
   (   23.1000   ,    3.0807   )
   (   23.2000   ,    3.0853   )
   (   23.3000   ,    3.0899   )
   (   23.4000   ,    3.0944   )
   (   23.5000   ,    3.0989   )
   (   23.6000   ,    3.1034   )
   (   23.7000   ,    3.1079   )
   (   23.8000   ,    3.1123   )
   (   23.9000   ,    3.1168   )
   (   24.0000   ,    3.1212   )
   (   24.1000   ,    3.1256   )
   (   24.2000   ,    3.1300   )
   (   24.3000   ,    3.1343   )
   (   24.4000   ,    3.1387   )
   (   24.5000   ,    3.1430   )
   (   24.6000   ,    3.1473   )
   (   24.7000   ,    3.1516   )
   (   24.8000   ,    3.1559   )
   (   24.9000   ,    3.1601   )
   (   25.0000   ,    3.1644   )
   (   25.1000   ,    3.1686   )
   (   25.2000   ,    3.1728   )
   (   25.3000   ,    3.1769   )
   (   25.4000   ,    3.1811   )
   (   25.5000   ,    3.1852   )
   (   25.6000   ,    3.1894   )
   (   25.7000   ,    3.1935   )
   (   25.8000   ,    3.1976   )
   (   25.9000   ,    3.2017   )
   (   26.0000   ,    3.2057   )
   (   26.1000   ,    3.2098   )
   (   26.2000   ,    3.2138   )
   (   26.3000   ,    3.2178   )
   (   26.4000   ,    3.2218   )
   (   26.5000   ,    3.2258   )
   (   26.6000   ,    3.2297   )
   (   26.7000   ,    3.2337   )
   (   26.8000   ,    3.2376   )
   (   26.9000   ,    3.2415   )
   (   27.0000   ,    3.2454   )
   (   27.1000   ,    3.2493   )
   (   27.2000   ,    3.2532   )
   (   27.3000   ,    3.2570   )
   (   27.4000   ,    3.2609   )
   (   27.5000   ,    3.2647   )
   (   27.6000   ,    3.2685   )
   (   27.7000   ,    3.2723   )
   (   27.8000   ,    3.2761   )
   (   27.9000   ,    3.2799   )
   (   28.0000   ,    3.2836   )
   (   28.1000   ,    3.2874   )
   (   28.2000   ,    3.2911   )
   (   28.3000   ,    3.2948   )
   (   28.4000   ,    3.2985   )
   (   28.5000   ,    3.3022   )
   (   28.6000   ,    3.3059   )
   (   28.7000   ,    3.3095   )
   (   28.8000   ,    3.3132   )
   (   28.9000   ,    3.3168   )
   (   29.0000   ,    3.3204   )
   (   29.1000   ,    3.3240   )
   (   29.2000   ,    3.3276   )
   (   29.3000   ,    3.3312   )
   (   29.4000   ,    3.3348   )
   (   29.5000   ,    3.3383   )
   (   29.6000   ,    3.3419   )
   (   29.7000   ,    3.3454   )
   (   29.8000   ,    3.3489   )
   (   29.9000   ,    3.3524   )
   (   30.0000   ,    3.3559   )
   (   30.1000   ,    3.3594   )
   (   30.2000   ,    3.3629   )
   (   30.3000   ,    3.3663   )
   (   30.4000   ,    3.3698   )
   (   30.5000   ,    3.3732   )
   (   30.6000   ,    3.3766   )
   (   30.7000   ,    3.3800   )
   (   30.8000   ,    3.3834   )
   (   30.9000   ,    3.3868   )
   (   31.0000   ,    3.3902   )
   (   31.1000   ,    3.3936   )
   (   31.2000   ,    3.3969   )
   (   31.3000   ,    3.4003   )
   (   31.4000   ,    3.4036   )
   (   31.5000   ,    3.4069   )
   (   31.6000   ,    3.4102   )
   (   31.7000   ,    3.4135   )
   (   31.8000   ,    3.4168   )
   (   31.9000   ,    3.4201   )
   (   32.0000   ,    3.4233   )
   (   32.1000   ,    3.4266   )
   (   32.2000   ,    3.4298   )
   (   32.3000   ,    3.4331   )
   (   32.4000   ,    3.4363   )
   (   32.5000   ,    3.4395   )
   (   32.6000   ,    3.4427   )
   (   32.7000   ,    3.4459   )
   (   32.8000   ,    3.4491   )
   (   32.9000   ,    3.4523   )
   (   33.0000   ,    3.4554   )
   (   33.1000   ,    3.4586   )
   (   33.2000   ,    3.4617   )
   (   33.3000   ,    3.4648   )
   (   33.4000   ,    3.4680   )
   (   33.5000   ,    3.4711   )
   (   33.6000   ,    3.4742   )
   (   33.7000   ,    3.4773   )
   (   33.8000   ,    3.4804   )
   (   33.9000   ,    3.4834   )
   (   34.0000   ,    3.4865   )
   (   34.1000   ,    3.4896   )
   (   34.2000   ,    3.4926   )
   (   34.3000   ,    3.4956   )
   (   34.4000   ,    3.4987   )
   (   34.5000   ,    3.5017   )
   (   34.6000   ,    3.5047   )
   (   34.7000   ,    3.5077   )
   (   34.8000   ,    3.5107   )
   (   34.9000   ,    3.5137   )
   (   35.0000   ,    3.5166   )
   (   35.1000   ,    3.5196   )
   (   35.2000   ,    3.5226   )
   (   35.3000   ,    3.5255   )
   (   35.4000   ,    3.5285   )
   (   35.5000   ,    3.5314   )
   (   35.6000   ,    3.5343   )
   (   35.7000   ,    3.5372   )
   (   35.8000   ,    3.5401   )
   (   35.9000   ,    3.5430   )
   (   36.0000   ,    3.5459   )
   (   36.1000   ,    3.5488   )
   (   36.2000   ,    3.5517   )
   (   36.3000   ,    3.5545   )
   (   36.4000   ,    3.5574   )
   (   36.5000   ,    3.5602   )
   (   36.6000   ,    3.5631   )
   (   36.7000   ,    3.5659   )
   (   36.8000   ,    3.5687   )
   (   36.9000   ,    3.5715   )
   (   37.0000   ,    3.5743   )
   (   37.1000   ,    3.5771   )
   (   37.2000   ,    3.5799   )
   (   37.3000   ,    3.5827   )
   (   37.4000   ,    3.5855   )
   (   37.5000   ,    3.5883   )
   (   37.6000   ,    3.5910   )
   (   37.7000   ,    3.5938   )
   (   37.8000   ,    3.5965   )
   (   37.9000   ,    3.5993   )
   (   38.0000   ,    3.6020   )
   (   38.1000   ,    3.6047   )
   (   38.2000   ,    3.6074   )
   (   38.3000   ,    3.6101   )
   (   38.4000   ,    3.6128   )
   (   38.5000   ,    3.6155   )
   (   38.6000   ,    3.6182   )
   (   38.7000   ,    3.6209   )
   (   38.8000   ,    3.6236   )
   (   38.9000   ,    3.6262   )
   (   39.0000   ,    3.6289   )
   (   39.1000   ,    3.6315   )
   (   39.2000   ,    3.6342   )
   (   39.3000   ,    3.6368   )
   (   39.4000   ,    3.6394   )
   (   39.5000   ,    3.6421   )
   (   39.6000   ,    3.6447   )
   (   39.7000   ,    3.6473   )
   (   39.8000   ,    3.6499   )
   (   39.9000   ,    3.6525   )
   (   40   ,    3.6551   )
};
